Insights from the Field: Exploring Students' Perspectives on Bad Unit Testing Practices

Educating students about software testing practices is integral to the curricula of many computer science-related courses and typically involves students writing unit tests. Similar to production/source code, students might inadvertently deviate from established unit testing best practices, and introduce problematic code, referred to as test smells, into their test suites. Given the extensive catalog of test smells, it becomes challenging for students to identify test smells in their code, especially for those who lack experience with testing practices. In this experience report, we aim to increase students' awareness of bad unit testing practices, and detail the outcomes of having 184 students from three higher educational institutes utilize an IDE plugin to automatically detect test smells in their code. Our findings show that while students report on the plugin's usefulness in learning about and detecting test smells, they also identify specific test smells that they consider harmless. We anticipate that our findings will support academia in refining course curricula on unit testing and enabling educators to support students with code review strategies of test code.

==> assets/table-notharmful.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table}[]
% \caption{Frequency and reasoning of smells considered non-harmful by participants}
% \label{Table:nonharmful}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lcl@{}}
% \toprule
% \multicolumn{1}{c}{\textbf{Test Name}} & \textbf{Frequency} & \multicolumn{1}{c}{\textbf{Reason for why it is non-harmful}}                                                                                                                                                                                                                                                                                                                                                                                                    \\ \midrule
% Lazy Test                              & 81                 & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not affect the correctness or functionality of the test results.\\ - Does not introduce any errors or issues.\\ - In projects of small size used in assignment, lazy test do not pose a significant concern.\\ - Does not compromise code line coverage, and all test cases pass successfully.\\ - Does not provide meaningful coverage of the code.\\ - False positive\end{tabular} \\ \midrule
% Magic Number Test                      & 49                 & \begin{tabular}[c]{@{}l@{}}- Does not affect the correctness or functionality of the test results.\\ - Does not introduce any errors or issues.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                  \\ \midrule
% Eager Test                             & 31                 & \begin{tabular}[c]{@{}l@{}}- Does not affect the correctness or functionality of the test results.\\ - Does not introduce any errors or issues.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                  \\ \midrule
% Empty Test                             & 19                 & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not affect the correctness or functionality of the test results.\\ - Does not compromise code line coverage; all test cases pass successfully.\end{tabular}                                                                                                                                                                                                                          \\ \midrule
% Duplicate Assert                       & 17                 & \begin{tabular}[c]{@{}l@{}}- Does not affect the correctness or functionality of the test results.\\ - Makes code shorter and enhance overall efficiency\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                         \\ \midrule
% Redundant Print                        & 16                 & - No impact on the ease of maintenance.                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
% Ignored Test                           & 15                 & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                                                                                               \\ \midrule
% Verbose Test                           & 14                 & - No impact on the ease of maintenance.                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
% Redundant Assertion                    & 12                 & - No experience                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \midrule
% Assertion Roulette                     & 12                 & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not affect the correctness or functionality of the test results.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                     \\ \midrule
% Constructor Initialization             & 11                 & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not introduce any errors or issues.\end{tabular}                                                                                                                                                                                                                                                                                                                                     \\ \midrule
% Default Test                           & 11                 & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not introduce any errors or issues.\end{tabular}                                                                                                                                                                                                                                                                                                                                     \\ \midrule
% Unknown Test                           & 10                 & - No impact on the ease of maintenance.                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
% General Fixture                        & 9                  & - Does not affect the correctness or functionality of the test results.                                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
% Conditional Test Logic                 & 9                  & - False positive                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
% Exception Handling                     & 9                  & - False positive                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
% Mystery Guest                          & 9                  & - No reasons provided                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \midrule
% Sensitive Equality                     & 8                  & \begin{tabular}[c]{@{}l@{}}- No experience\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                       \\ \midrule
% Sleepy Test                            & 8                  & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                                                                                               \\ \midrule
% Resource Optimism                      & 8                  & - No experience                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \bottomrule
% \end{tabular}%
% }
% \end{table}




\begin{table}[]
\caption{Frequency and reasoning of smells considered non-harmful by participants}
\label{Table:nonharmful}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{1}{c}{\textbf{Test Name}} & \multicolumn{1}{c}{\textbf{Reason for why it is non-harmful}}                                                                                                                                                                                                                                                                                                                                                                                                    \\ \midrule
Lazy Test                              & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not affect the correctness or functionality of the test results.\\ - Does not introduce any errors or issues.\\ - In projects of small size used in assignment, lazy test do not pose a significant concern.\\ - Does not compromise code line coverage, and all test cases pass successfully.\\ - Does not provide meaningful coverage of the code.\\ - False positive\end{tabular} \\ \midrule
Magic Number Test                      & \begin{tabular}[c]{@{}l@{}}- Does not affect the correctness or functionality of the test results.\\ - Does not introduce any errors or issues.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                  \\ \midrule
Eager Test                            & \begin{tabular}[c]{@{}l@{}}- Does not affect the correctness or functionality of the test results.\\ - Does not introduce any errors or issues.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                  \\ \midrule
Empty Test                            & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not affect the correctness or functionality of the test results.\\ - Does not compromise code line coverage; all test cases pass successfully.\end{tabular}                                                                                                                                                                                                                          \\ \midrule
Duplicate Assert                       & \begin{tabular}[c]{@{}l@{}}- Does not affect the correctness or functionality of the test results.\\ - Makes code shorter and enhance overall efficiency\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                         \\ %\midrule Redundant Print                        & - No impact on the ease of maintenance.                                                                                                                                                                                                                                                                                                                                                                                                                          \\ %\midrule Ignored Test                           & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                                                                                               \\ %\midrule Verbose Test                           & - No impact on the ease of maintenance.                                                                                                                                                                                                                                                                                                                                                                                                                          \\ %\midrule Redundant Assertion                    & - No experience                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ %\midrule Assertion Roulette                     & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not affect the correctness or functionality of the test results.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                     %\\ \midrule Constructor Initialization             & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not introduce any errors or issues.\end{tabular}                                                                                                                                                                                                                                                                                                                                     \\ %\midrule Default Test                           & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - Does not introduce any errors or issues.\end{tabular}                                                                                                                                                                                                                                                                                                                                     \\ %\midrule Unknown Test                           & - No impact on the ease of maintenance.                                                                                                                                                                                                                                                                                                                                                                                                                          \\ %\midrule General Fixture                        & - Does not affect the correctness or functionality of the test results.                                                                                                                                                                                                                                                                                                                                                                                          \\ % \midrule Conditional Test Logic                 & - False positive                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ %\midrule Exception Handling                     & - False positive                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ %\midrule Mystery Guest                          & - No reasons provided                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ %\midrule Sensitive Equality                     & \begin{tabular}[c]{@{}l@{}}- No experience\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                       \\ %\midrule Sleepy Test                            & \begin{tabular}[c]{@{}l@{}}- No impact on the ease of maintenance.\\ - False positive\end{tabular}                                                                                                                                                                                                                                                                                                                                                               \\ %\midrule Resource Optimism                      & - No experience                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\
\bottomrule
\end{tabular}%
}
\end{table}

==> temp.tex <==


Unit testing is an industry-standard software engineering technique that involves writing small, self-contained tests to verify the correctness of individual code units. Unit testing is the basic building block of software testing, and therefore the Association for Computing Machinery (ACM) recommends the integration of unit testing in Computer Science and Software Engineering curricula\footnote{https://www.acm.org/education/curricula-recommendations}. Consequently, seeking educational practices for teaching software testing is becoming the focus of various researchers, resulting in a Software Testing Education Workshop\footnote{https://testedworkshop.github.io/2023/}. 

These studies focus on designing appropriate pedagogical methods of teaching unit test programming and identifying appropriate testing frameworks that can be adopted for educational purposes. Yet, little is known about how to assess the non-functional quality of students' tests, in order to avoid bad programming practices in their test code. Bad programming practices in test code, also known as \textit{test smells}, are indicators of potential design problems in the test suite. Test smells are similar to code smells, which are bad programming practices in production code. The existence of test smells negatively impact the system's testing performance, by increasing the flakiness of test cases, and hindering test code readability and understandability.

Prior research has correlated the prevalence of test smells with developers' deviation from adopting best practices of writing test code, such as X-Unit \cite{meszaros2007xunit}. Therefore, it is critical to raise awareness of test smells among students (prospective developers) and to provide them with the tools and training needed to write high-quality test code.

